Region-based semantic segmentation with end-to-end training

We propose a novel method for semantic segmentation, the task of labeling each pixel in an image with a semantic class. Our method combines the advantages of the two main competing paradigms. Methods based on region classification offer proper spatial support for appearance measurements, but typically operate in two separate stages, none of which targets pixel labeling performance at the end of the pipeline. More recent fully convolutional methods are capable of end-to-end training for the final pixel labeling, but resort to fixed patches as spatial support. We show how to modify modern region-based approaches to enable end-to-end training for semantic segmentation. This is achieved via a differentiable region-to-pixel layer and a differentiable free-form Region-of-Interest pooling layer. Our method improves the state-of-the-art in terms of class-average accuracy with 64.0% on SIFT Flow and 49.9% on PASCAL Context, and is particularly accurate at object boundaries.

==> sec-discussion.tex <==
\section{To be removed/merged: Discussion}
In this section we discuss the advantages and disadvantages of our method with respect to the used region proposals and different loss functions.

\jasper{I'm not sure this section is necessary. I'd rather have these arguments in the
experiments.}
\holger{Okay, let's integrate them above.}

\subsection{Region proposals}

Although region proposals have proven to be beneficial in many applications~\cite{}, they are subject to frequent criticism.
Note that our method is not limited to any region proposal algorithm, but in Sec. superpixelmodel we achieve significant speedups for bottom-up proposal methods.
Several works mention region proposal computation as a bottleneck at test time~\cite{ren15nips}.
Therefore Faster R-CNN~\cite{ren15nips} introduce a Region Proposal Network that shares convolutional features with the detection network and enables nearly cost-free region proposals.
Future work will focus on the integration of Region Proposal Networks into our method.
\holger{Mention Dollar's proposals}
\jasper{Yes, Dollar should be mentioned somewhere.
Maybe in conclusion, or a mini-discussion paragraph.}

\subsection{Evaluation criterion and loss function}
% Pix-acc
Early semantic segmentation works~\cite{} use global pixel accuracy as evaluation criterion.
Due to the region-to-pixel layer presented in Sec.~\ref{sec:endtoend}, we are able to compute an accurate pixel-level loss that corresponds to global pixel accuracy.
This is how we achieve state-of-the-art results on pixel accuracy on SIFT Flow in Table~\ref{tab:experiments-siftflow}.
\jasper{We already said this. Redundant.}

% Class-pix acc
Works that focus on rare and small object classes use the class-average pixel accuracy criterion~\cite{}. %cite tighe %used in VOC2007 segmentation task
We can optimize for this criterion using a class-weighted loss as shown in Sec.~\ref{sec:rareclasses}.
In Table~\ref{tab:experiments-siftflow} and~\ref{tab:experiments-pascalcontext} we show that we outperform the state-of-the-art on class-average pixel accuracy by $9\%$ and $5\%$ on SIFT Flow and PASCAL Context respectively.
\jasper{We already said this. Redundant.}

% Mean IOU
The most recent criterion is mean Intersection over Union~(mIoU).  %used from VOC2008 segmentation task % has been used on instances in object detection
This measure presented in~\cite{everingham10ijcv} for semantic segmentation penalizes high false-positive rates, making the per-class results more meaningful.
We present promising results PASCAL Context with the mIoU measure in Table~\ref{tab:experiments-pascalcontext}.
We observe that our method tends to spatially overshoot on rare classes~(i.e. classifying the entire sky as bird), achieving previously unseen class-average pixel accuracy at the cost of slightly decreased mean IOU.
Cogswell et al.~\cite{cogswell14arxiv} show how to maximize mIoU by minimizing Union over Intersection for a given mini-batch.
This loss function can be directly applied to our pixel-level softmax outputs to optimize mIoU in an end-to-end fashion.
We assume that this would further improve our results on the mIoU criterion.
\jasper{Bold claims. Our mIoU scores are, objectively, not promising at all.}

